On the Hardness of Robustness Transfer: A Perspective from Rademacher Complexity over Symmetric Difference Hypothesis Space

Recent studies demonstrated that the adversarially robust learning under $\ell_\infty$ attack is harder to generalize to different domains than standard domain adaptation. How to transfer robustness across different domains has been a key question in domain adaptation field. To investigate the fundamental difficulty behind adversarially robust domain adaptation (or robustness transfer), we propose to analyze a key complexity measure that controls the cross-domain generalization: the adversarial Rademacher complexity over {\em symmetric difference hypothesis space} $\mathcal{H} \Delta \mathcal{H}$. For linear models, we show that adversarial version of this complexity is always greater than the non-adversarial one, which reveals the intrinsic hardness of adversarially robust domain adaptation. We also establish upper bounds on this complexity measure. Then we extend them to the ReLU neural network class by upper bounding the adversarial Rademacher complexity in the binary classification setting. Finally, even though the robust domain adaptation is provably harder, we do find positive relation between robust learning and standard domain adaptation. We explain \emph{how adversarial training helps domain adaptation in terms of standard risk}. We believe our results initiate the study of the generalization theory of adversarially robust domain adaptation, and could shed lights on distributed adversarially robust learning from heterogeneous sources, e.g., federated learning scenario.

==> Notations.tex <==
\section{Notations \llv{no need to be a separate section. put it at the beginning of problem setup}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> classification_lower_bound.tex <==
\section{Linear Classification: Lower Bound}
\begin{theorem}
For any monotone non-increasing classification loss function that satisfies $\phi(x) = 0 \forall x \geq 1$, e.g., 0-1 loss or hinge loss, and assume that $\exists \bw \in \mathcal{W}, |\bw^\top \bx_i| - \epsilon \|\bw\|_1 \geq 1, \forall i \in [n]$ , we have:
 \begin{align*}
    \hat{\Re}_\cD (\tilde{\ell}\circ \cH \Delta \cH) \geq  \hat{\Re}_\cD ({\ell}\circ \cH \Delta \cH)
\end{align*}
\begin{proof}
\begin{align*}
    \hat{\Re}_\cD (\tilde{\ell}\circ \cH \Delta \cH) = \mathbb{E}_\sigma \left[\sup_{\bw,\bw':\|\bw\|_p\leq W, \|\bw'\|_p \leq W} \frac{1}{n}\sum_{i=1}^n \sigma_i \max_{\|\boldsymbol{\delta}\|_\infty \leq \epsilon} \left|\text{Sgn}(\bw^\top (\bx_i + \boldsymbol{\delta})) - \text{Sgn}(\bw'^\top (\bx_i + \boldsymbol{\delta}))\right|\right]
\end{align*}
Let $v_i (\bw,\bw'):= \max_{\|\boldsymbol{\delta}\|_\infty \leq \epsilon} \left|\text{Sgn}(\bw^\top (\bx_i + \boldsymbol{\delta})) - \text{Sgn}(\bw'^\top (\bx_i + \boldsymbol{\delta}))\right|$, and $\bv := [v_1,...,v_n]$. We denote the range of $\|\bv\|_p$ when $\|\bw\|_p\leq W, \|\bw'\|_p \leq W$ as $\cV:=\{\|\bv(\bw,\bw')\|_p: \bw,\bw':\|\bw\|_p\leq W, \|\bw'\|_p \leq W \}$, and we assume $\cV = [0,V^+]$. We notice that the left end $0$ is reachable if we choose $\bw = \bw'$.
 
 

So we re-write the above adversarial Rademacher as:
\begin{align*}
    \hat{\Re}_\cD (\tilde{\ell}\circ \cH \Delta \cH) = \mathbb{E}_\sigma \left[\sup_{\bv: \|\bv\|_p \in [0,V^+]} \frac{1}{n}\sum_{i=1}^n \sigma_i  v_i\right] = \frac{V^+}{n}\mathbb{E}_\sigma \left\| \boldsymbol{\sigma}  \right\|_q.
\end{align*}

Similarly, Let $u_i (\bw,\bw'):= \left|\text{Sgn}(\bw^\top\bx_i) - \text{Sgn}(\bw'^\top \bx_i )\right|$, and $\bu := [u_1,...,u_n]$. We denote the range of $\|\bu\|_p$ when $\|\bw\|_p\leq W, \|\bw'\|_p \leq W$ as $\cU:=\{\|\bu(\bw,\bw')\|_p: \bw,\bw':\|\bw\|_p\leq W, \|\bw'\|_p \leq W \}$, and we assume $\cU = [U^-,U^+]$ where $0 \leq U^- \leq U^+$. We can rewrite Rademacher complexity under standard loss as:
\begin{align*}
   \hat{\Re}_\cD ( {\ell}\circ \cH \Delta \cH) \leq  \mathbb{E}_\sigma \left[\sup_{\bu: \|\bu\|_p \in [0,U^+]} \frac{1}{n}\sum_{i=1}^n \sigma_i  u_i\right] = \frac{U^+}{n}\mathbb{E}_\sigma \left\| \boldsymbol{\sigma}  \right\|_q. 
\end{align*}
 We know that $V^+ \geq U^+$ due to the max operator in adversarial Rademacher. Since $U^+ \leq V^+$, we must have $\hat{\Re}_\cD ( {\ell}\circ \cH \Delta \cH) \leq \hat{\Re}_\cD (\tilde{\ell}\circ \cH \Delta \cH)$.
\end{proof}


\end{theorem}

==> draft_attempts.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Classification loss: Other attempts}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Ref: \cite{burer2009nonconvex}.

\nid{*** begining ***

July 13th: I suggest that before relaxing the problem, you write it as a Quadratic Program:}
Let $\mW \eqdef \bw \bw'^\top$,
\begin{eqnarray*}
    &\min_{\mQ \in \R^{p \times p}, \ \bdelta \in \R^d} &\mathbf{Tr}(\mQ \mW) + \bx^\top (\mW^\top + \mW) \bdelta + \bx^T \mW \bx\\
    &\text{subject to} \ & \mathbf{e}_i^T \bdelta -\epsilon \leq 0, \quad \forall i \in [p],\\
    && - \mathbf{e}_i^T \bdelta -\epsilon \leq 0, \quad \forall i \in [p],\\
    && \mQ = \bdelta \bdelta^T
\end{eqnarray*}
since easy computations give that $\mathbf{Tr}(\mQ \mW) = \mathbf{Tr}(\bdelta \bdelta^\top \bw \bw'^\top) = \bdelta^\top \bw \bw'^\top  \bdelta$.
\nid{*** end ***}
For lower bound, we consider the following convex relaxation. Let $\mathbf{W} = \mathbf{w}\mathbf{w}'^T$, and then we have the following SDP relaxation:
\begin{eqnarray*}
    &\min_{\mathbf{Q}, \boldsymbol{\delta}} &\mathbf{Tr}(\mathbf{Q}\mathbf{W}) + \boldsymbol{\delta}^T \mathbf{W} \mathbf{x}+ \mathbf{x} \mathbf{W} \boldsymbol{\delta} + \mathbf{x}^T \mathbf{W} \mathbf{x}\\
    &\text{subject to} \ & \mathbf{e}_i^T \boldsymbol{\delta} -\epsilon \leq 0, \forall i \in [d],\\
    && \mathbf{Q} \succeq \boldsymbol{\delta}\boldsymbol{\delta}^T
\end{eqnarray*}
\nid{July 13th: I would rather use $\mD$ instead of $\mQ$ ($\mD$ or $\Delta$ like Delta $\bdelta$)

- Q1) isn't $\mA$ the same matrix as $\mW?

- Q2) Don't you miss the $p$ constraints $-\delta_i \leq \epsilon$ ?
}

Using Schur complement, we can rewrite the constraint and get:
\begin{eqnarray*}
    &\min_{\mathbf{Q}\in \mathbb{R}^{d\times d}, \boldsymbol{\delta} \in \mathbb{R}^d} \ &\mathbf{Tr}(\mathbf{Q}\mathbf{W}) + \bx^\top (\mW^\top + \mW) \bdelta  + \mathbf{x}^T \mathbf{W} \mathbf{x}\\
    &\text{Subject to:} \  &\mathbf{e}_i^T \boldsymbol{\delta} -\epsilon \leq 0, \forall i \in [d],\\
    &&- \mathbf{e}_i^T \bdelta -\epsilon \leq 0, \quad \forall i \in [d],\\
    &&\begin{bmatrix} 
 \mathbf{Q} & \boldsymbol{\delta}\\
 \boldsymbol{\delta}^T & 1 
\end{bmatrix} \succeq  0
\end{eqnarray*}
\paragraph{Trial 1:}

Assuming $\mQ$ is positive semidefinite (PSD) (is it still a relaxation ?), we let $\mathbf{z} = \mathbf{Q}^{-\frac{1}{2}}\boldsymbol{\delta}$, then we can rewrite the definiteness constraint as:
\begin{align*}
    \begin{bmatrix} 
 \mathbf{Q} & \boldsymbol{\delta}\\
 \boldsymbol{\delta}^T & 1 
\end{bmatrix}  =  \begin{bmatrix} 
 \mathbf{Q}^{\frac{1}{2}} & \boldsymbol{0}\\
 \boldsymbol{0}^T & 1 
\end{bmatrix}  \begin{bmatrix} 
 \mathbf{I} & \mathbf{z}\\
 \mathbf{z}^T & 1 
\end{bmatrix}  \begin{bmatrix} 
 \mathbf{Q}^{\frac{1}{2}} & \boldsymbol{0}\\
 \boldsymbol{0}^T & 1 
\end{bmatrix} \succeq 0 
\end{align*}
We can drop left and right matrices and the relation still holds:
\begin{align*}
  \begin{bmatrix} 
 \mathbf{I} & \mathbf{z}\\
 \mathbf{z}^T & 1 
\end{bmatrix}  \succeq 0  \iff \|\mathbf{z}\| \leq 1.
\end{align*}
\nid{July 13th: to double check}
So the SDP can be rewritten as:
\begin{eqnarray*}
    &\min_{\mathbf{Q} \in S_{+}^d, \mathbf{z}} \ &\mathbf{Tr}(\mathbf{Q}\mathbf{W}) + (\mathbf{Q}^{\frac{1}{2}}\mathbf{z})^T \mathbf{W} \mathbf{x}+ \mathbf{x} \mathbf{W} \mathbf{Q}^{\frac{1}{2}}\mathbf{z} + \mathbf{x}^T \mathbf{A} \mathbf{x}\\
    &\text{Subject to:} \  &\mathbf{e}_i^T \mathbf{Q}^{\frac{1}{2}}\mathbf{z} -\epsilon \leq 0, \forall i \in [d],\\
    &&\|\mathbf{z}\| \leq 1
\end{eqnarray*}

\paragraph{Trial 2:} Using KKT condition:
    The Lagrangian:
\begin{align*}
    \mathcal{L}(\mathbf{Q},\boldsymbol{\delta}, \boldsymbol{\mu},\boldsymbol{\nu},\mathbf{Z}) = \mathbf{Tr}(\mathbf{Q}\mathbf{W}) + \bx^\top (\mW^\top + \mW) \bdelta + \mathbf{x}^T \mathbf{W} \mathbf{x} +\sum_{i=1}^d {\mu}_i (\mathbf{e}_i^T \boldsymbol{\delta} - {\epsilon}) +\sum_{i=1}^d  {\nu}_i (-\mathbf{e}_i^T \boldsymbol{\delta} - {\epsilon}) - \left\langle \begin{bmatrix} 
 \mathbf{Q} & \boldsymbol{\delta}\\
 \boldsymbol{\delta}^T & 1 
\end{bmatrix}, \mathbf{Z} \right \rangle
\end{align*}
where
\begin{align*}
    \mathbf{Z} = \begin{bmatrix} 
 \mathbf{S} & \mathbf{u}\\
 \mathbf{u}^T & s 
\end{bmatrix}
\end{align*}

Taking the derivative w.r.t. each of four variables:
\begin{align*}
    &\frac{\partial \mathcal{L}}{\partial \mathbf{Q}} = \mathbf{W} - \frac{\partial tr(  
 \mathbf{Q} \mathbf{S}+\boldsymbol{\delta} \mathbf{u}^T) +\boldsymbol{\delta}^T\mathbf{u}+s}{\partial \mathbf{Q}} = \mathbf{W} - \mathbf{S} = 0\\ 
  &\frac{\partial \mathcal{L}}{\partial \bdelta} = (\mW^\top + \mW)\bx + \sum_{i=1}^d {\mu}_i \mathbf{e}_i^T   -\sum_{i=1}^d  {\nu}_i \mathbf{e}_i^T  - \frac{\partial tr(  
 \mathbf{Q} \mathbf{S}+\boldsymbol{\delta} \mathbf{u}^T) +\boldsymbol{\delta}^T\mathbf{u}+s}{\partial \bdelta} =(\mW^\top + \mW)\bx + \sum_{i=1}^d {\mu}_i \mathbf{e}_i^T   -\sum_{i=1}^d  {\nu}_i \mathbf{e}_i^T - 2\mathbf{u} = 0
\end{align*}
primal feasibility:
\begin{align*}
     \mathbf{e}_i^T \boldsymbol{\delta} - {\epsilon} \leq 0,\\
 -\mathbf{e}_i^T \boldsymbol{\delta} - {\epsilon} \leq 0.
\end{align*}
dual feasibility:
\begin{align*}
    \mu_i \geq 0, \nu_i \geq 0, \mathbf{Z} \succeq 0.
\end{align*}
complementary slackness:
\begin{align*}
    \sum_{i=1}^d {\mu}_i (\mathbf{e}_i^T \boldsymbol{\delta} - {\epsilon}) = 0,\\
    \sum_{i=1}^d  {\nu}_i (-\mathbf{e}_i^T \boldsymbol{\delta} - {\epsilon}) = 0,\\
    -\left\langle \begin{bmatrix} 
 \mathbf{Q} & \boldsymbol{\delta}\\
 \boldsymbol{\delta}^T & 1 
\end{bmatrix}, \mathbf{Z} \right \rangle = 0.
\end{align*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Maybe junk: QP reformulation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nid{I think this* is not a Quadratically Constrained Quadratic Program (QCQP) but rather a simpler Quadratic Program (QP) as the constraints are linear.}
We consider the problem*
\begin{eqnarray}
    \label{eq:quadratic_program}
    \min_{\bdelta \in \R^p : \|\bdelta\|_\infty\leq \epsilon} (\bx_i+\bdelta)^\top \bw \bw'^\top (\bx_i+\bdelta) 
    = \underbrace{\bx_i^\top \mQ \bx_i}_{\text{kept as we are interested in the function value}} \ + &\min_{\bdelta \in \R^p} & \bdelta^T \mQ \bdelta + \bc^\top \bdelta\\
    &\text{subject to: } & 
    \mA
    \bdelta \preceq \bb \nonumber
\end{eqnarray}
where we defined $\mQ \eqdef \bw \bw'^\top \in \R^{p \times p}$, $\bc \eqdef (\mQ+ \mQ^\top) \bx \in \R^p$, $\mA \eqdef \begin{bmatrix} \mI_p \\ -\mI_p \end{bmatrix} \in \R^{2p \times p}$, $\bb \eqdef \epsilon \begin{bmatrix} \bfone_p \\ -\bfone_p \end{bmatrix} \in \R^p$ and $\preceq$ is an component-wise inequality sign.

\nid{Maybe we can separate the optimization over the orthogonal component of $\bw$ and $\bw'$ respectively, depending wheteher they are orthognal.}

This problem in~\eqref{eq:quadratic_program} is NOT exactly a Quadratic Program (QP), with ($2p$) linear constraints as described in 
\url{https://en.wikipedia.org/wiki/Quadratic_programming#Problem_formulation}.

Concerning the almost QP in~\eqref{eq:quadratic_program}, we can find 
\begin{itemize}
    \item an \textbf{upper-bound} by taking a particular point
    \item a \textbf{lower-bound} by taking looking at the dual and finding an upper-bound of it (might be hard to find a feasible point for the dual)    
\end{itemize}

The dual of the QP is given by 
\begin{eqnarray}
    \label{eq:dual_quadratic_program}
    &\max_{\bdelta \in \R^p} & -\frac{1}{2} \lambda^\top \mA \mQ^{-1} \mA^\top - \lambda^\top b \\
    &\text{subject to: } & \lambda \geq 0 \nonumber
\end{eqnarray}
as written in \url{https://en.wikipedia.org/wiki/Quadratic_programming#Lagrangian_duality}.
\nid{Problem: $\mQ = \bw \bw'^\top$ is not invertible, not even symmetric...
Maybe we can symmetrize it by writing $\mQ = \underbrace{\mQ + \mQ^\top}_{\text{symmetric}} - \mQ^\top$
}

==> impact.tex <==
\section*{Broader Impact}
This work advocates a distributionally robust algorithm for federated learning. The algorithmic solution is designed to preserve the privacy of users, while trains a high quality model. The proposed algorithm tries to minimize the maximum loss among distributions (clients' data). Hence, we can ensure that even if the data distribution among users is highly heterogeneous the trained model is reasonably good for everyone, and not benefiting only a group of clients. This will ensure the fairness in training a global model with respect to every user, and it is vitally important for critical decision making systems such as healthcare. In such a scenario, the model learned by simple algorithms such as FedAvg would have an inconsistent performance over different distributions, which is not acceptable. However, the resulting model from our algorithm will have robust performance over different distributions it has been trained on.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

